Detecting High-Energy Neutrino Minibursts from Local Supernovae with Multiple Neutrino Observatories

Growing evidence from multi-wavelength observations of extragalactic supernovae (SNe) has established the presence of dense circumstellar material in Type II SNe. Interaction between the SN ejecta and the circumstellar material should lead to diffusive shock acceleration of cosmic rays and associated high-energy emission. Observation of high-energy neutrinos along with the MeV neutrinos from SNe will provide unprecedented opportunities to understand unanswered questions in cosmic-ray and neutrino physics. We show that current and future neutrino detectors can identify high-energy neutrinos from an extragalactic SN in the neighborhood of the Milky Way. We present the prospects for detecting high-energy neutrino minibursts from SNe in known local galaxies, and demonstrate how the network of multiple high-energy neutrino detectors will extend the horizon for the identification of high-energy SN neutrinos. We also discuss high-energy neutrino emission from SN 2023ixf.

==> jdefs.tex <==
% Bibliography and bibfile
\def\lnp{Lec.\ Notes in Physics}
          % Lecture Notes in Physics
\def\cpc{Comp.\ Phys.\ Comm.}
          % Computer Physics Communications
\def\jpg{J. Phys. G}
          % Journal of Physics G Nuclear Physics
\def\ijmpa{Int.\ J.\ Mod.\ Phys.\ A}
          % International Journal of Modern Physics A
\def\epjc{Eur.\ Phys.\ J.\ C}
          % European Physical Journal C
\def\nima{Nuc.\ Inst.\ Methods A}
          % Nuclear Instruments and Methods A
\def\nimb{Nuc.\ Inst.\ Methods B}
          % Nuclear Instruments and Methods B
\def\njp{New J.\ Phys.}
          % New Journal of Physics
\def\rmp{Rev.\ Mod.\ Phys.}
          % Reviews of Modern Physics
\def\app{Astropart.\ Phys.}
          % Astroparticle Physics
\def\aj{AJ}%
          % Astronomical Journal
\def\actaa{Acta Astron.}%
          % Acta Astronomica
\def\araa{ARA\&A}%
          % Annual Review of Astron and Astrophys
\def\arnps{Ann.~Rev.~Nucl.~\& Part.~Sci.}%
          % Annual Review of Astron and Astrophys
\def\apj{ApJ}%
          % Astrophysical Journal
\def\apjl{ApJ}%
          % Astrophysical Journal, Letters
\def\apjs{ApJS}%
          % Astrophysical Journal, Supplement
\def\ao{Appl.\ Opt.}%
          % Applied Optics
\def\apss{Ap\&SS}%
          % Astrophysics and Space Science
\def\aap{A\&A}%
          % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}%
          % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}%
          % Astronomy and Astrophysics, Supplement
\def\azh{AZh}%
          % Astronomicheskii Zhurnal
\def\pos{PoS}%
          % Proceedings of Science
\def\baas{BAAS}%
          % Bulletin of the AAS
\def\bac{Bull.\ Astr.\ Inst.\ Czechosl.}%
          % Bulletin of the Astronomical Institutes of Czechoslovakia 
\def\caa{Chinese Astron.\ Astrophys.}%
          % Chinese Astronomy and Astrophysics
\def\cjaa{Chinese J.\ Astron.\ Astrophys.}%
          % Chinese Journal of Astronomy and Astrophysics
\def\icarus{Icarus}%
          % Icarus
\def\jhep{JHEP}%
          % Journal of High Energy Physics
\def\jcap{JCAP}%
          % Journal of Cosmology and Astroparticle Physics
\def\jpsj{J.\ Phys.\ Soc.\ Japan}%
          % Journal of the Physical Society of Japan
\def\jrasc{JRASC}%
          % Journal of the RAS of Canada
\def\canjphys{Can.~J.~Phys.}
          %Canadian Journal of Physics
\def\apphys{Astropart.~Phys.}
          %Astroparticle Physics
\def\mnras{MNRAS}%
          % Monthly Notices of the RAS
\def\memras{MmRAS}%
          % Memoirs of the RAS
\def\na{New A}%
          % New Astronomy
\def\nar{New A Rev.}%
          % New Astronomy Review
\def\pasa{PASA}%
          % Publications of the Astron. Soc. of Australia
\def\pra{Phys.\ Rev.\ A}%
          % Physical Review A: General Physics
\def\prb{Phys.\ Rev.\ B}%
          % Physical Review B: Solid State
\def\prc{Phys.\ Rev.\ C}%
          % Physical Review C
\def\prd{Phys.\ Rev.\ D}%
          % Physical Review D
\def\pre{Phys.\ Rev.\ E}%
          % Physical Review E
\def\prl{Phys.\ Rev.\ Lett.}%
          % Physical Review Letters
\def\pasp{PASP}%
          % Publications of the ASP
\def\pasj{PASJ}%
          % Publications of the ASJ
\def\qjras{QJRAS}%
          % Quarterly Journal of the RAS
\def\rmxaa{Rev. Mexicana Astron. Astrofis.}%
          % Revista Mexicana de Astronomia y Astrofisica
\def\skytel{S\&T}%
          % Sky and Telescope
\def\solphys{Sol.\ Phys.}%
          % Solar Physics
\def\sovast{Soviet~Ast.}%
          % Soviet Astronomy
\def\ssr{Space~Sci.\ Rev.}%
          % Space Science Reviews
\def\zap{ZAp}%
          % Zeitschrift fuer Astrophysik
\def\nat{Nature}%
          % Nature
\def\science{Science}%
\def\sci{\science}%
          % Science
\def\iaucirc{IAU~Circ.}%
          % IAU Cirulars
\def\aplett{Astrophys.\ Lett.}%
          % Astrophysics Letters
\def\apspr{Astrophys.\ Space~Phys.\ Res.}%
          % Astrophysics Space Physics Research
\def\bain{Bull.\ Astron.\ Inst.\ Netherlands}%
          % Bulletin Astronomical Institute of the Netherlands
\def\fcp{Fund.\ Cosmic~Phys.}%
          % Fundamental Cosmic Physics
\def\gca{Geochim.\ Cosmochim.\ Acta}%
          % Geochimica Cosmochimica Acta
\def\grl{Geophys.\ Res.\ Lett.}%
          % Geophysics Research Letters
\def\jcp{J.\ Chem.\ Phys.}%
          % Journal of Chemical Physics
\def\jgr{J.\ Geophys.\ Res.}%
          % Journal of Geophysics Research
\def\jqsrt{J.\ Quant.\ Spec.\ Radiat.\ Transf.}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\def\memsai{Mem.\ Soc.\ Astron.\ Italiana}%
          % Mem. Societa Astronomica Italiana
\def\nphysa{Nucl.\ Phys.\ A}%
          % Nuclear Physics A
\def\nphysb{Nucl.\ Phys.\ B}%
          % Nuclear Physics B
\def\physrep{Phys.\ Rep.}%
          % Physics Reports
\def\physscr{Phys.\ Scr}%
          % Physica Scripta
\def\planss{Planet.\ Space~Sci.}%
          % Planetary Space Science
\def\procspie{Proc.\ SPIE}%
          % Proceedings of the SPIE
\def\repprogphys{Rep.\ Prog.\ Phys.}%
          % Reports of Progress in Physics
\def\jpcrd{J. Phys. Chem. Ref. Data}% 
        %Journal of Physical and Chemical Reference Data 
\def\jphysb{J. Phys. B}% 
	%Journal of Physics B Atomic Molecular Physics
\def\jphysd{J. Phys. D}% 
	%Journal of Physics D
\def\jphysconfseries{J. Phys. Conf. Series}% 
	%Journal of Physics: Conference Series
\def\physrev{\pr}
\def\pr{Phys. Rev.}% 
	%Physical Review
\def\josa{J. Opt. Soc. Amer. (1917-1983)}% 
	%Journal of the Optical Society of America (1917-1983) 
\def\josab{J. Opt. Soc. Amer. B}% 
	%Journal of the Optical Society of America B Optical Physics
\def\pla{Phys. Lett. A}% 
	%Physics Letters A
\def\plb{Phys. Lett. B}% 
	%Physics Letters B
\def\os{Opt. Spectrosc. (Russ.)}% 
	%Optics and Spectroscopy (Russ. / USSR)
\def\jas{J. Appl. Spectrosc.}% 
	%Journal of Applied Spectroscopy (Russ. / USSR)
\def\annp{Ann. Phys.}% 
	%Annalen der Physik
\def\sa{Spectrochim. Acta}% 
	%Spectrochimica Acta
\def\prsoca{Proc. R. Soc. London Ser. A}% 
	%Proceedings of the Royal Society of London, Series A
\def\zphysa{Z. Phys. A}% 
	%Zeitschrift fur Physik A
\def\zphysb{Z. Phys. B}% 
	%Zeitschrift fur Physik B
\def\zphysc{Z. Phys. C}% 
	%Zeitschrift fur Physik C
\def\zphysd{Z. Phys. D}% 
	%Zeitschrift fur Physik D
\def\zphyse{Z. Phys. E}% 
	%Zeitschrift fur Physik E
\def\zphys{Z. Phys.}% 
	%Zeitschrift fur Physik
\def\adndt{Atom. Data Nuc. Data Tables}% 
	%Atomic Data and Nuclear Data Tables
\def\jmolspec{J. Mol. Spectrosc.}% 
	%Journal of Molecular Spectroscopy
\def\aphysb{Appl. Phys. B}% 
	%Applied Physics B: Lasers and Optics
\def\nim{Nuc. Inst. Meth.}% 
	%Nuclear Instruments and Methods
\def\jphysique{J. Phys. (Paris)}% 
	%Journal de Physique
\def\epjp{Eur.~Phys.~J.~Plus}%
        %European Phhysical Journal Plus
\def\epjc{Eur.~Phys.~J.~C}%
        %European Phhysical Journal C
\def\njp{New J.~Phys.}
        %New Journal of Physics
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao
%

